Conways game of life as an analogue to a habitable world Livingness beyond the biological

Conways Game of Life is a cellular automaton noted for its rich, complex, and emergent behavior, which seems qualitatively lifelike it exists within a wider space of different rule-sets of cellular automata none of which have been found to display behaviors that seem as rich as Conways selected example We present here a set of three quantitative tests for lifelike behavior based on the critical brain theory Shannons theory of information entropy and integrated information theory all of which are successfully able to select Conways Game of Life as an outlier within this set which is a nonbiological analogue to the selection of a habitable planet or universe among a wider space of similar settings that cannot support the same kinds of living systems

==> Figs.tex <==
\input{IAU_Sample}
